Causal Abstractions of Neural Networks

Structural analysis methods (e.g., probing and feature attribution) are increasingly important tools for neural network analysis. We propose a new structural analysis method grounded in a formal theory of causal abstraction that provides rich characterizations of model-internal representations and their roles in input/output behavior. In this method, neural representations are aligned with variables in interpretable causal models, and then interchange interventions are used to experimentally verify that the neural representations have the causal properties of their aligned variables. We apply this method in a case study to analyze neural models trained on Multiply Quantified Natural Language Inference (MQNLI) corpus, a highly complex NLI dataset that was constructed with a tree-structured natural logic causal model. We discover that a BERT-based model with state-of-the-art performance successfully realizes parts of the natural logic model's causal structure, whereas a simpler baseline model fails to show any such structure, demonstrating that BERT representations encode the compositional structure of MQNLI.

==> Figures/interchangeresults.tex <==
\begin{tikzpicture}
  \centering
  \pgfplotsset{every tick label/.append style={font=\scriptsize}}
  \begin{axis}[
        ybar, axis on top,
        title={ \small Examples in Subset (Out of 500)},
        height=8cm, width=16.7cm,
        bar width=0.1cm,
        ymajorgrids, tick align=inside,
        ymin=0, ymax=500,
        axis x line*=bottom,
        y axis line style={opacity=100},
        tickwidth=0pt,
        legend style={
            at={(0.5,-0.1)},
            anchor=north,
            legend columns=-1,
            /tikz/every even column/.append style={column sep=0.5cm}
        },
        % y label style = {at={(axis description cs:0.05,0.5)}},
        symbolic x coords={ 
        $Q_{Subj}$,
        $Q_{Obj}$,
        $Neg$,
        $Adj_{Subj}$,
        $N_{Subj}$,
        $Adv$,
        $V$,
        $Adj_{Obj}$,
        $N_{Obj}$,
        $NP_{Subj}$,
        $VP$,
        $NP_{Obj}$,
        $QP_{Obj}$,
        $NegP$
        },
       xtick=data,
       nodes near coords={
        \pgfmathprintnumber[precision=0]{\pgfplotspointmeta}
       }
    ]
    \addplot [draw=none, fill=blue!40] coordinates {
        ($Q_{Subj}$,100)
        ($Q_{Obj}$,93)
        ($Neg$, 160)
        ($Adj_{Subj}$, 193)
        ($N_{Subj}$, 408)
        ($Adv$,231 )
        ($V$, 156 )
        ($Adj_{Obj}$,167 )
        ($N_{Obj}$, 428 )
        ($NP_{Obj}$, 157)
        ($VP$, 220)
        ($NP_{Subj}$, 187)
        ($QP_{Obj}$, 100)
        ($NegP$,68)
      };
   \addplot [draw=none,fill=red!40] coordinates {
        ($Q_{Subj}$,56)
           ($Q_{Obj}$,37)
        ($Neg$, 7)
        ($Adj_{Subj}$, 119)
        ($N_{Subj}$,28)
        ($Adv$,17)
        ($V$, 5)
        ($Adj_{Obj}$, 16 )
        ($N_{Obj}$, 0)
        ($NP_{Obj}$,55)
        ($VP$,72)
        ($NP_{Subj}$,115 )
        ($QP_{Obj}$, 50)
        ($NegP$,8)
   };
   \addplot [draw=none, fill=green!40] coordinates {
        ($Q_{Subj}$,2)
           ($Q_{Obj}$,5)
        ($Neg$, 2)
        ($Adj_{Subj}$, 0 )
        ($N_{Subj}$,0 )
        ($Adv$,2 )
        ($V$,0 )
        ($Adj_{Obj}$,0 )
        ($N_{Obj}$,0 )
        ($NP_{Obj}$,0 )
        ($VP$,2 )
        ($NP_{Subj}$,0 )
        ($QP_{Obj}$,2 )
        ($NegP$,2 )
   };

    \legend{BERT,LSTM,Random Baseline}
  \end{axis}
  \end{tikzpicture}

==> Figures/tokentable.tex <==
\begin{tabular}{|c|c|}
        $Q_{Obj}$ & $[CLS], Q^P_{Obj}, Q^H_{Subj}$\\
        $Q_{Subj}$ & $[CLS],Q^P_{Subj}, Q^H_{Obj}$\\
        $Neg$ & $[CLS],Neg^P, Neg^H$\\
        $Adj_{Subj}$ & $[CLS],Adj_{Subj}^P,Adj^H_{Subj}$\\
        $N_{Subj}$ & $[CLS],N_{Subj}^P,N^H_{Subj}$\\
        $Adv$ & $[CLS],Adv^P, Adv^H$\\
        $V$ & $[CLS],V^P, V^H$\\
        $Adj_{Obj}$ & $[CLS],Adj_{Obj}^P,Adj^H_{Obj}$\\
        $N_{Obj}$ & $[CLS],N_{Obj}^P,N^H_{Obj}$\\
        $NP_{Obj}$ & $[CLS],N_{Obj}^P,N^H_{Obj}$\\
        $VP$\\
        $NP_{Subj}$\\
        $QP_{Obj}$\\
        $NegP$\\
\end{tabular}

==> Tables/mqnli-examples-aligned.tex <==
% \begin{table*}[htp]
%   \centering
%   \renewcommand{\arraystretch}{1}
%   \begin{tabular}[c]{ p{0.4\textwidth} c  p{0.4\textwidth} }
%     \toprule
%     Premise & Relation & Hypothesis \\
%     \midrule
%     $\varepsilon$ every $\varepsilon$ baker $\varepsilon$ $\varepsilon$ $\varepsilon$ eats $\varepsilon$ no $\varepsilon$ bread
%     & contradiction
%     & $\varepsilon$ no angry baker $\varepsilon$ $\varepsilon$ $\varepsilon$ eats $\varepsilon$ no $\varepsilon$ bread
%     \\
%     $\varepsilon$ every silly professor $\varepsilon$ $\varepsilon$ $\varepsilon$ sells not every $\varepsilon$ book 
%     & neutral
%     & $\varepsilon$ every silly professor $\varepsilon$ $\varepsilon$ $\varepsilon$ sells not every $\varepsilon$ chair 
%     \\
%     not every happy professor $\varepsilon$ $\varepsilon$ fairly admits not every unusual idea
%     & entailment
%     & $\varepsilon$ some $\varepsilon$ professor does not $\varepsilon$ admits $\varepsilon$ no $\varepsilon$ idea
%     \\
%     \bottomrule
%   \end{tabular}
\begin{table}[t]
\begin{subtable}[t]{0.5\textwidth}
\centering
\fontsize{8.2pt}{8.2pt}\selectfont
\begin{tabular}
 $\varepsilon$ every $\varepsilon$ baker $\varepsilon$ $\varepsilon$ $\varepsilon$ eats $\varepsilon$ no $\varepsilon$ bread \\
\textbf{contradiction} \\
$\varepsilon$ no angry baker $\varepsilon$ $\varepsilon$ $\varepsilon$ eats $\varepsilon$ no $\varepsilon$ bread \\
\\
$\varepsilon$ every silly professor $\varepsilon$ $\varepsilon$ $\varepsilon$ sells not every $\varepsilon$ book \\
\textbf{neutral}\\
$\varepsilon$ every silly professor $\varepsilon$ $\varepsilon$ $\varepsilon$ sells not every $\varepsilon$ chair \\
\\
not every happy professor $\varepsilon$ $\varepsilon$ fairly admits not every odd idea \\
\textbf{entailment} \\
$\varepsilon$ some $\varepsilon$ professor does not $\varepsilon$ admits $\varepsilon$ no $\varepsilon$ idea 
\end{tabular}    

 \caption{MQNLI examples. The $\varepsilon$ token ensures a perfect alignment between both premises and hypotheses and across all examples. It is semantically an identity element.}
  \label{tab:mqnli-examples}
  \end{subtable}
  \hfill
  \begin{subtable}[t]{0.45\textwidth}
  \centering
  \begin{tabular}{l c c c}
    \toprule
    Model &  Train & Dev & Test\\
    \midrule
    CBoW       & 88.04 & 54.18 & 53.99 \\
    TreeNN     & 67.01 & 54.01 & 53.73 \\
    CompTreeNN & 99.65 & 80.17 & 80.21 \\[0.25ex]
    BiLSTM     & 99.42 & 46.41 & 46.32 \\
    BERT       & 99.99 & \textbf{88.25} & \textbf{88.50} \\
    \bottomrule
  \end{tabular}
  \caption{MQNLI results. The first three models are from \citealt{Geiger-etal:2019}, where the CompTreeNN is task-specific model not suitable for general NLI and functions as an idealized upperbound. Our results show that BERT-based models can surpass this without such alignments.}
  \label{tab:accuracy}
  \end{subtable}
    \caption{MQNLI examples (left) and MQNLI results (right).}
\end{table}
